Implications of Distance over Redistricting Maps: Central and Outlier Maps

In representative democracy, a redistricting map is chosen to partition an electorate into districts which each elects a representative. A valid redistricting map must satisfy a collection of constraints such as being compact, contiguous, and of almost-equal population. However, these constraints are loose enough to enable an enormous ensemble of valid redistricting maps. This enables a partisan legislature to gerrymander by choosing a map which unfairly favors it. In this paper, we introduce an interpretable and tractable distance measure over redistricting maps which does not use election results and study its implications over the ensemble of redistricting maps. Specifically, we define a central map which may be considered "most typical" and give a rigorous justification for it by showing that it mirrors the Kemeny ranking in a scenario where we have a committee voting over a collection of redistricting maps to be drawn. We include running time and sample complexity analysis for our algorithms, including some negative results which hold using any algorithm. We further study outlier detection based on this distance measure and show that our framework can detect some gerrymandered maps. More precisely, we show some maps that are widely considered to be gerrymandered that lie very far away from our central maps in comparison to a large ensemble of valid redistricting maps. Since our distance measure does not rely on election results, this gives a significant advantage in gerrymandering detection which is lacking in all previous methods.

==> Acks.tex <==
\section{Acknowledgments}
We would like to thank Daniel Smolyak for helpful discussions and the UMD CS Department for providing computational resources. 

==> new_experiments.tex <==
\section{Numerical Results for Special Maps on the Distance Histogram}
%\begin{table}[h]
%\caption{Percentile distances for special maps in NC using the unweighted distance measure.} \label{table:nc_unweighted_distances}
%\begin{center}
%\begin{tabular}{lll}
%\textbf{NC} & \textbf{Judge's Map} & \textbf{2016 enacted map} & \textbf{2011 enacted map} \\
%\hline \\
%Seed 1        & xxxxxx &   xx   &            \ \ \ \ \ \ \ \ \ \ \ \ xxxxxx  \\
%Seed 2         & xxxxxx &   xx     &  \ \ \ \ \ \ \ \ \ \ \ \ xxxxxx   \\
%Seed 3        & xxxxxx &         xxx  &        \ \ \ \ \ \ \ \ \ \ \ \ xxxxxx  \\
%\end{tabular}
%\end{center}
%\end{table}


% NC: unweighted distance table  
\begin{table}[h!]
\caption{Percentile distances for special maps in NC using the unweighted distance measure.} \label{table:nc_unweighted_distances}
\begin{center}
\begin{tabular}{*{4}{c}}
\textbf{Starting Seed} & \textbf{Judges' map} & \textbf{2016 enacted map} & \textbf{2011 enacted map} \\
\hline \\
Seed 1         & 49.472 &                  99.944    &	 100.\\
Seed 2         &  50.676 &         	       99.931     &	 100\\
Seed 3         & 53.761 &                  99.949    & 	100\\
\end{tabular}
\end{center}
\end{table}


% NC: distance table  
\begin{table}[h!]
\caption{Percentile distances for special maps in NC using the weighted distance measure.} \label{table:nc_weighted_distances}
\begin{center}
\begin{tabular}{*{4}{c}}
\textbf{Starting Seed} & \textbf{Judges' map} & \textbf{2016 enacted map} & \textbf{2011 enacted map} \\
\hline \\
Seed 1         & 58.070 &                  99.998    &	 100.\\
Seed 2         &  59.846 &         	       99.991     &	100.\\
Seed 3         & 62.738&                  99.998    & 	100.\\
\end{tabular}
\end{center}
\end{table}




% PA: unweighted distance table  
\begin{table}[h!]
\caption{Percentile distances for special maps in PA using the unweighted distance measure.} \label{table:pa_unweighted_distances}
\begin{center}
\begin{tabular}{*{3}{c}}
\textbf{Starting Seed} & \textbf{Remedial map} & \textbf{2011 enacted map} \\
\hline \\
Seed 1         & 43.864 &           100.    \\
Seed 2         &  45.238 &         	99.982   \\
Seed 3         &  43.787 &                  100.    \\
\end{tabular}
\end{center}
\end{table}


% PA: weighted distance table  
\begin{table}[h!]
\caption{Percentile distances for special maps in PA using the weighted distance measure.} \label{table:pa_weighted_distances}
\begin{center}
\begin{tabular}{*{3}{c}}
\textbf{Starting Seed} & \textbf{Remedial map} & \textbf{2011 enacted map} \\
\hline \\
Seed 1         & 18.147 &            100.    \\
Seed 2         &  18.433 &         	99.994    \\
Seed 3         & 17.743 &                 100.    \\
\end{tabular}
\end{center}
\end{table}


\section{Are the Medoids More Competetive?}


%%% 1-NC unweighted medoids 
%%%\begin{figure}\label{fig:NC_med_unweighted_elections}
%%%\centering
%%%\begin{subfigure}
%%%   \includegraphics[width=1\linewidth]{Marked_unweighted_PA_election_histograms_all_2.png}
%%%\end{subfigure}

%%%\begin{subfigure}
%%%   \includegraphics[width=1\linewidth]{Marked_unweighted_PA_election_histograms_all_2.png}
%%%\end{subfigure}

%%%\begin{subfigure}
%%%   \includegraphics[width=1\linewidth]{Marked_unweighted_PA_election_histograms_all_2.png}
%%%\end{subfigure}
%%%\caption[Elections in the unweighted NC medoids.}
%%%\end{figure}


% 1-NC unweighted medoids 
\begin{figure}
  \centering
  \subfloat[All Medoids]{\includegraphics[scale=0.3]{NC_unweighted_election_percentages.png} \label{fig:a}} \\
  % \subfloat[Seed 2 Medoid]{\includegraphics[scale=0.3]{Marked_unweighted_PA_election_histograms_all_2.png} \label{fig:b}} \\
  %  \subfloat[Seed 3 Medoid]{\includegraphics[scale=0.3]{Marked_unweighted_PA_election_histograms_all_2.png} \label{fig:c}} 
  \caption{Percentage election results in the unweighted NC medoids.} \label{fig:AB}
\end{figure}


% 2-NC weighted medoids 
\begin{figure}
  \centering
  \subfloat[All Medoids]{\includegraphics[scale=0.3]{NC_weighted_election_percentages.png} \label{fig:a}} \\
  % \subfloat[Seed 2 Medoid]{\includegraphics[scale=0.3]{Marked_unweighted_PA_election_histograms_all_2.png} \label{fig:b}} \\
  %  \subfloat[Seed 3 Medoid]{\includegraphics[scale=0.3]{Marked_unweighted_PA_election_histograms_all_2.png} \label{fig:c}} 
  \caption{Percentage election results in the weighted NC medoids.} \label{fig:AB}
\end{figure}


% 3-MD unweighted medoids 
\begin{figure}
  \centering
  \subfloat[All Medoids]{\includegraphics[scale=0.3]{MD_unweighted_election_percentages.png} \label{fig:a}} \\
  % \subfloat[Seed 2 Medoid]{\includegraphics[scale=0.3]{Marked_unweighted_PA_election_histograms_all_2.png} \label{fig:b}} \\
  %  \subfloat[Seed 3 Medoid]{\includegraphics[scale=0.3]{Marked_unweighted_PA_election_histograms_all_2.png} \label{fig:c}} 
  \caption{Percentage election results in the unweighted MD medoids.} \label{fig:AB}
\end{figure}


% 4-MD weighted medoids 
\begin{figure}
  \centering
  \subfloat[All Medoids]{\includegraphics[scale=0.3]{MD_weighted_election_percentages.png} \label{fig:a}} \\
  % \subfloat[Seed 2 Medoid]{\includegraphics[scale=0.3]{Marked_unweighted_PA_election_histograms_all_2.png} \label{fig:b}} \\
  %  \subfloat[Seed 3 Medoid]{\includegraphics[scale=0.3]{Marked_unweighted_PA_election_histograms_all_2.png} \label{fig:c}} 
  \caption{Percentage election results in the weighted MD medoids.} \label{fig:AB}
\end{figure}


% 5-PA unweighted medoids 
\begin{figure}
  \centering
  \subfloat[All Medoids]{\includegraphics[scale=0.3]{PA_unweighted_election_percentages.png} \label{fig:a}} \\
  % \subfloat[Seed 2 Medoid]{\includegraphics[scale=0.3]{Marked_unweighted_PA_election_histograms_all_2.png} \label{fig:b}} \\
  %  \subfloat[Seed 3 Medoid]{\includegraphics[scale=0.3]{Marked_unweighted_PA_election_histograms_all_2.png} \label{fig:c}} 
  \caption{Percentage election results in the unweighted PA medoids.} \label{fig:AB}
\end{figure}


% 6-PA weighted medoids 
\begin{figure}
  \centering
  \subfloat[All Medoids]{\includegraphics[scale=0.3]{PA_weighted_election_percentages.png} \label{fig:a}} \\
  % \subfloat[Seed 2 Medoid]{\includegraphics[scale=0.3]{Marked_unweighted_PA_election_histograms_all_2.png} \label{fig:b}} \\
  %  \subfloat[Seed 3 Medoid]{\includegraphics[scale=0.3]{Marked_unweighted_PA_election_histograms_all_2.png} \label{fig:c}} 
  \caption{Percentage election results in the weighted PA medoids.} \label{fig:AB}
\end{figure}




%Experimentally, we test our results over the states of North Carolina, Maryland, and Pennsylvania. Interestingly, we find that a by product of having a central map is a method for detecting gerrymandered maps. Concretely, the states of North Carolina and Pennsylvania have had enacted maps which were widely considered to be gerrymandered and in fact some were struck down by the state supreme court \cite{LWVPenn2018}. In response, some remedial maps were either suggested or enacted. We find that when we sample a large ensemble of redistricting maps and plot their distances from the centroid map, the gerrymandered maps have very large distances at the tail of the distribution whereas the remedial maps are much closer to the centroid. This is a non-trivial progress in detecting gerrymandered maps since the previous methods consistently relied on election results while we only need a distance measure. This also perhaps suggests a new rule in drawing redistricting maps. Specifically, the drawn map should not be too faraway from the centroid. 



% We introduce the novel approach of choosing a \emph{central} map among a set of redistricting maps and propose a method for identifying such a map. More concretely, we define a family of metrics over redistricting maps and give a linear time algorithm that can find the medoid of a collection of given maps. Moreover, under the assumption that we can sample valid maps in an independent and identically distributed fashion, we derive the sample complexity for obtaining the \emph{centroid} redistricting map. Further, we demonstrate that a gerrymandered map can be far from this centroid in practice even when the distance metric does not explicitly use partisan features.



% The metric space we focus on in this work represents a map as an adjacency matrix on the voting units (blocks). Two units are considered ``adjacent'' in a given map if that map puts them in the same district. Choosing a central map in this space means we are more likely to place a subset of units in the same district if they are often placed in the same district across many maps in the collection. When the collection is generated by random sampling, then many voters who would likely be in the same district on average if a random map was drawn will end up in the same district in our chosen central map. This is related to the concepts of pairwise fairness and community preservation advanced in~\cite{brubach2020pairfair} as measures of fairness to individual voters and communities rather than fairness to political parties. 
% Although our experimental results suggest our method also produces maps which are more fair to political parties, our primary goal is fairness to voters with respect to the political geography of a state, and we note that many practical reform efforts favor avoiding the use of partisan information while drawing the maps.


% While we focus on a specific metric here, most aspects of the general approach we propose are flexible enough to be applied to other metric spaces. 
% For example, voting history and partisan data could easily be incorporated to emphasize partisan fairness more if state constitutions were changed to require this. 
% Our approach could also be extended to the problem of choosing a map from among a collection of maps submitted by citizens.\footnote{Some states and governors have piloted this type of citizen map submission approach. Of course, sampling guarantees would not apply in this case. In addition, consideration would need to be given to strategic map submissions such as users spamming the system with a desired map.} 
% % (of course, sampling guarantees would not apply in this case). 
% We discuss this situation of citizens submitting maps more in the next section.


% \subsection{Connections to Other Redistricting Reforms}


% Among the current most prominent directions of reform in the process of drawing new redistricting maps are the introduction of redistricting commissions and involvement of citizens in the redistricting process. Redistricting commissions have now been adopted in some form by several states although in some cases, the legislature retains final control.
% Often called ``independent'' commissions, they are typically designed to be non-partisan or balanced in their partisan make-up. 

% More recently, many state governments, redistricting commissions, and academic researchers have begun soliciting map submissions from engaged citizens through online platforms. This type of citizen engagement in redistricting can take many forms. For example, redistricting is still controlled by the state legislature in Maryland, one of the two states at the center of the U.S. Supreme Court case Rucho v. Common Cause~\cite{CaseRucho2019}. Nevertheless, an independent redistricting commission formed by an executive order from the governor has established a web page to collect citizen submissions of redistricting plans~\cite{MDProposalsProcess}. To further facilitate this process, a web portal using the Maptitude software was set up to allow anyone to draw a map~\cite{MDMaptitude}. Other commonly-used free web apps for drawing redistricting maps include DistrictR~\cite{Districtr} from the Metric Geometry and Gerrymandering Group (MGGG) and the DRA 2020 app~\cite{DavesRedistricting} from Dave's Redistricting. 

% The Maryland Citizens Redistricting Commission page states:
% \begin{quotation}
%     Drawing new boundaries for Maryland's congressional and state legislative districts is not an activity reserved for the Maryland Citizens Redistricting Commission (Commission) alone. You can do it too. 
    
    
%     The Commission accepts and welcomes input and recommendations from the public via public hearings and has posted tools on its website that will allow anyone with a computer to recommend what new districts should look like.
% \end{quotation}

% As of this writing, the Maryland site features 83 citizen submissions including both congressional and legislative maps~\cite{MDProposalsSubmissions}. It remains to be seen whether this process will be viewed as a serious effort to solicit citizen input or a political stunt by a governor whose political party would gain from even a non-partisan map versus one drawn by the state legislature controlled by the other party. This tension highlights the need for more transparent and well-studied methods to analyze a set of maps and find a compromise or central map.



% social media platforms like twitter


% Further, it is clear that there is in fact a collection of maps that can be considered valid, had that not been the case then the sampling techniques introduced would be meaningless since there is only one unique redistricting map. 

















